The Adversarial Consistency of Surrogate Risks for Binary Classification

We study the consistency of surrogate risks for robust binary classification. It is common to learn robust classifiers by adversarial training, which seeks to minimize the expected $0$-$1$ loss when each example can be maliciously corrupted within a small ball. We give a simple and complete characterization of the set of surrogate loss functions that are \emph{consistent}, i.e., that can replace the $0$-$1$ loss without affecting the minimizing sequences of the original adversarial risk, for any data distribution. We also prove a quantitative version of adversarial consistency for the $\rho$-margin loss. Our results reveal that the class of adversarially consistent surrogates is substantially smaller than in the standard setting, where many common surrogates are known to be consistent.

==> Sections/background_old.tex <==
\section{Problem Setup}\label{sec:problem_setup}
\subsection{Surrogate Risks}\label{sec:surrogate_risks}
This paper studies binary classification on $\Rset^d$. Explicitly, labels are $\{-1,+1\}$ and the data is distributed according to a distribution $\cD$ on the set $\Rset^d\times\{-1,+1\}$. The measures $\PP_1$, $\PP_0$ define the probabilities of finding points with a given label in a region of $\Rset^d$. Formally, define measures on $\Rset^d$ by
\[\PP_1(A)=\cD(A\times \{+1\}), \PP_0(A)=\cD(A\times \{-1\}).\]
%Throughout this paper, we assume that 
%\begin{assumption}\label{as:absolute_cont}
%    $\PP_1,\PP_0$ are absolutely continuous with respect to Lebesgue measure.
%\end{assumption}

Typical classification algorithms involve learning a real-valued function $f$ and then classifying according to the sign of $f$, which we define as 
\[\sgn \alpha =\begin{cases} +1 &\text{if } \alpha> 0\\ -1&\text{if } \alpha\leq 0\end{cases}.\]
The choice $\sgn 0=-1$ is arbitrary. The \emph{classification risk} $R(f)$ is then the probability of misclassifying a point under $\cD$; $R(f)=\cD(\sgn f(\bx) \neq y)$. The classification risk in terms of the marginal distributions $\PP_0,\PP_1$ is
\begin{equation}\label{eq:standard_zero_one_loss}
    R(f)= \int\one_{f(\bx)\leq 0}d\PP_1+\int  \one_{f(\bx)> 0} d\PP_0.    
\end{equation}



%One can also think of a classifier as a set; the points $A(f)=\{\bx\colon f(\bx)>0\}$ are classified as $+1$ and $A(f)^C=\{ \bx\colon f(\bx)\leq 0\}$ is classified as $-1$. 



%While describing the adversarial classification problem, we will find it more convenient to specify a classifier by the set $A(f)$ rather than the function $f$. 

In the adversarial setting, every $x$-value is perturbed by a malicious adversary before undergoing classification by $f$. We assume that these perturbations are bounded by $\e$ in some norm $\|\cdot\|$ and furthermore, the adversary knows both our classifier $f$ and the true label of the point $\bx$. In the machine learning literature, this attack model is called the \emph{evasion attack}. 
In other words, $f$ misclassifies $\bx$ when there is a point $\bx'\in \ov{B_\e(\bx)}$ for which $\sgn f(\bx')\neq y$. Hence, a point $\bx$ with label $+1$ is misclassified when there is a point $\|\bx'-\bx\|\leq \e$ for which $f(\bx')\leq 0$ and a point $\bx$ with label $-1$ is misclassified when there is a point $\|\bx'-\bx\|\leq \e$ for which $f(\bx')> 0$. 
Therefore, the expected fraction of errors made by the classifier $f$ under this model is therefore
Conveniently, this criterion can be expressed in terms of supremums. 
Mathematically, for any function $g$, we define
\begin{equation*}
    S_\e(g)(\bx)=\sup_{\|\bh\|\leq \e} g(\bx+\bh)
\end{equation*}
A point $\bx$ with label $+1$ is misclassified when $S_\e(\one_{f\leq 0}))=1$ and a point $\bx$ with label $-1$ is misclassified when $S_\e(\one_{f> 0}=1$. Hence the adversarial analog of the classification risk is
\begin{align}
    R^\e(f)&= \int S_\e(\one_{f\leq 0})d\PP_1+\int  S_\e(\one_{f>0}) d\PP_0, \label{eq:adv_zero_one_loss_sup}
\end{align}
which is called the \emph{adversarial classification risk} \footnote{Defining this integral requires some care because for a Borel function $g$, $S_\e(g)$ may not be measurable; see Section~3.3 and Appendix~A of \citep{Frank2022Existence} details}.

Next, we discuss surrogate risks for the standard classification problem. In general, optimizing the empirical version of the classification risk is an intractable problem \citep{BenDavidEironLong2003}. Instead, we consider minimizing the risk
\begin{equation}\label{eq:standard_phi_loss}
    R_\phi(f)=\int \phi(f)d\PP_1+\int\phi(-f) d\PP_0
\end{equation}
over all measurable functions. A point $\bx$ is then classified according to $\sgn f$. There are many possible choices for $\phi$---typically one chooses a loss that is easy to optimize. In this paper, we assume that 
\begin{assumption}\label{as:phi}
    $\phi$ is non-increasing, non-negative, continuous, and $\lim_{\alpha\to \infty}\phi(\alpha)=0$.
\end{assumption}
 Most surrogate losses in machine learning satisfy this assumption. We call $R_\phi$ a \emph{consistent risk} and $\phi$ a \emph{consistent loss} if for all distributions, every minimizing sequence of $R_\phi$ is also a minimizing sequence of $R$.\footnote{In the context of standard (non-adversarial) learning, the concept we defined as consistency is often referred to as \emph{calibration}, see for instance \citep{BartlettJordanMcAuliffe2006,Steinwart2007}. We opt for the term `consistency' as the prior works \citep{AwasthiFrankMao2021,AwasthiMaoMohri,MeunierEttedguietal22} use calibration to refer to a different but related concept in the adversarial setting.} Consistent losses have been studied in many prior works; most prominently \citet{BartlettJordanMcAuliffe2006} showed that a convex decreasing loss $\phi$ is consistent iff $\phi$ is differentiable at zero and $\phi'(0)\neq 0$. 


Similarly, because optimizing \eqref{eq:adv_zero_one_loss_sup} is computationally intractable, one defines a surrogate for the adversarial classification risk \eqref{eq:adv_zero_one_loss_sup} by
\begin{align}
    &R_\phi^\e(f)=\int S_\e( \phi\circ fd\PP_1 +\int S_\e( \phi\circ -f(\bx'))d\PP_0\label{eq:adv_phi_loss}
\end{align}
Due to the supremum in this expression, we refer to this risk as a \emph{supremum-based surrogate}. We define adversarial consistency analogously. 
\begin{definition}
    Let $\PP_0,\PP_1$ define a data distribution. The loss $\phi$ is \emph{adversarially $\cH$-consistent} for $\PP_0,\PP_1$ if every sequence $h_n$ which minimizes $R_\phi^\e$ over $\cH$ also minimizes $R^\e$ over $\cH$. We say that $\phi$ is \emph{adversarially consistent} for $\PP_0,\PP_1$ if it is $\cH$-consistent for the class of all measurable functions. 
\end{definition}
    When referring to a loss as adversarially consistent, we will typically not specify $\PP_0,\PP_1$ as the data distribution should be clear from the context. 
    
    
    

    

We conclude by recalling a characterization of minimizers for $R_\phi$ and $R$ in the non-adversarial setting. %This characterization explains the presence of the extended real numbers in Lemmas~\ref{lemma:equivalent_defintions_standard} and~\ref{lemma:equivalent_definitions}.
 Finding minimizers of $R$ is straightforward -- by defining 
 \begin{equation}\label{eq:C_def}
    C(\eta,\alpha)=\eta \one_{f\leq 0}+(1-\eta) \one_{f>0},\quad C^*(\eta)=\inf_\alpha C(\eta,\alpha)
 \end{equation}
 $\PP=\PP_0+\PP_1,$ and $\eta=d\PP_1/d\PP$, one can write
\[R(f)=\int \eta(\bx) \one_{f(\bx)\leq 0}+(1-\eta(\bx))\one_{f(\bx)>0}d\PP=\int C(\eta(\bx),f(\bx))d\PP\]
Thus, $f$ minimizes $R$ so long as $f$ minimizes $C(\eta,\cdot)$ pointwise, or in other words, $C(\eta(\bx),f(\bx))=C^*(\eta(\bx))$ $\PP$-a.e. The same procedure finds minimizers of $R_\phi$. Let 
\begin{equation}\label{eq:C_phi_def}
    C_\phi(\eta,\alpha)\colon = \eta\phi(\alpha)+(1-\eta)\phi(-\alpha),\quad C_\phi^*(\eta)=\inf_\alpha C(\eta,\alpha) 
\end{equation}
In terms of $\eta$ and $\PP$, the loss $R_\phi$ is
\begin{equation}\label{eq:pw_loss}
    R_\phi(f)=\int C_\phi(\eta(\bx),f(\bx))d\PP    
\end{equation}
Thus $f$ is a minimizer of $R_\phi$ iff  $f$ minimizes $C_\phi(\eta(\bx),\alpha)$ $\PP$-a.e., or in other words, $C_\phi(\eta(\bx),f(\bx))=C_\phi^*(\eta))$ $\PP$-a.e. However, over the set $\Rset$, the function $C_\phi(\eta(\bx),\alpha)$ may not always have a minimizer; for instance consider the exponential loss $\psi(\alpha)=e^{-\alpha}$ at $\eta=1$. On the other hand, $C_\phi(\eta,\alpha)$ always has a minimizer in the extended real numbers $\ov \Rset\colon=\Rset \cup \{-\infty,+\infty\}$ due to the continuity of $\phi$. Therefore, in the remainder of this paper, we assume that functions $f$ assume values in $\ov \Rset$.
Note that integrals of functions assuming values in $\Rset\cup\{\infty\}$ can still be defined using standard measure theory, see for instance \citep{folland}. 

This alternative view of the risks $R$ and $R_\phi$ provides a pointwise criterion for consistency, which we prove in Appendix~\ref{app:alt_consistency_characterization}.

    \begin{theorem}\label{th:alt_consistency_characterization} %A loss $\phi$ is consistent iff every minimizer of $R_\phi$ is also a minimizer of $R$. 
    The following are equivalent:
    \begin{enumerate}
        \item $\phi$ is consistent
        \item \label{it:C_seq_background}Every minimizing sequence of $C_\phi(\eta,\cdot)$ is also a minimizing sequence of $C(\eta,\cdot)$
        \item \label{it:R_min_background}Every minimizer of $R_\phi$ is a minimizer of $R$
    \end{enumerate}
    \end{theorem}
    This result reduces studying minimizing sequences of functionals to studying minimizers of functions. We will show that \ref{it:C_seq_background} has an analog in the adversarial scenario but \ref{it:R_min_background} does not.


    \citet{MeunierEttedguietal22} show that Theorem~\ref{th:alt_consistency_characterization} does not hold in the adversarial setup.
    \begin{example}[\citep{MeunierEttedguietal22}]
    Let $\PP_0=\PP_1$ be the the uniform distribution on the unit ball $\ov{B_R(\zero)}$ and let $\e=2R$. Let $\phi$ be a continuous loss function for which $C_\phi^*(1/2)=\phi(0)$. Notice that $\inf_{f} R^\e(f)\geq \inf_f R(f)$ and $\inf_{f} R_\phi^\e(f)\geq \inf_f R_\phi(f)$. However, for the function $f^*\equiv 0$, $R^\e(f^*)=\inf_f R(f)=1/2$ and $R_\phi^\e(f^*)=\inf_f R_\phi(f)=\phi(0)$. Therefore $f^*$ minimizes both $R_\phi^\e$ and $R^\e$. Now consider the sequence of functions
    \[f_n(\bx)=\begin{cases} \frac 1n  &\bx=0\\
    -\frac 1n &\bx\neq 0\end{cases}\]
     Then $R_\phi^\e(f_n)=\phi(-1/n)$ while $R^\e(f_n)=1$ for all $n$. Thus $f_n$ is a minimizing sequence of $R_\phi^\e$ but not of $R^\e$.
    \end{example}
    Notice that all convex loss functions satisfy $C_\phi^*(1/2)=\phi(0)$.
    In this paper, we show prove that if $C_\phi^*(1/2)<\phi(0)$, then $\phi$ is adversarially consistent. This condition is equivalent to one studied in \citep{MeunierEttedguietal22}, namely that $0$ is not a minimizer of $C_\phi^*(1/2,\alpha)$. Some losses that satsify this property are the $\rho$-margin loss $\phi_rho(\alpha)=\min(1,\max( 1-\alpha/\rho,0))$ and the the shifted sigmoid loss proposed by \citep{MeunierEttedguietal22}, $\phi(\alpha)=1/(1+\exp(\alpha-\tau))$, $\tau>0$.


\subsection{Minimax Theorems for Adversarial Risks}\label{sec:existence_minimax}
    We study the consistency of $\phi$ by by comparing the minimizers of $R^\e_\phi$ with those of $R^\e$. 
        In the next section, in order to compare these minimizers, we will attempt to re-write the adversarial loss in a `pointwise' manner similar to \eqref{eq:pw_loss}. In order to achieve this representation of the adversarial loss, we apply minimax and complimentary slackness theorems from \citep{PydiJog2021,Frank2022Existence}. Before presenting these theorems, we introduce the $\infty$-Wasserstein metric from optimal transport. 
        For two measures $\QQ_0,\QQ_1$ satisfying $\QQ_0(\Rset^d)=\QQ_1(\Rset^d)$, let $\Pi(\QQ_0,\QQ_1)$ be the set of \emph{couplings} of $\QQ_0, \QQ_1$:
        \[\Pi(\QQ_0,\QQ_1)=\{ \gamma\colon \gamma(A\times \Rset^d)=\QQ_0(A), \gamma(\Rset^d\times A)=\QQ_1(A)\}\]
        
        The $W_\infty$ distance between $\QQ_0$ and $\QQ_1$ is defined as
    
        \[W_\infty(\QQ_0,\QQ_1)=\inf_{\gamma \in \Pi(\QQ_0,\QQ_1)} \esssup_{(\bx,\by)\sim \gamma} \|\bx-\by\| \]
        We denote the $\infty$-Wasserstein ball around a measure $\QQ$ by 
        \[\Wball \e (\QQ)=\{\QQ'\colon \QQ' \text{ Borel},\quad W_\infty(\QQ,\QQ')\leq \e \}\]
        Minimax theorems from prior work introduced dual problems to the adversarial classification risks \eqref{eq:adv_zero_one_loss_sup} and \eqref{eq:adv_phi_loss}. Let $\PP_0',\PP_1'$ be finite Borel measures and define
        \begin{equation}\label{eq:cdl_def}
            \cdl(\PP_0',\PP_1')=\int C^*\left(\frac{d \PP_1'}{d(\PP_0'+\PP_1')}\right)d(\PP_0'+\PP_1')
        \end{equation}
        where $C^*$ is defined by \eqref{eq:C_def}. The next theorem states that $\cdl$ optimized over $W_\infty$ balls is in fact a dual problem to $\cprm$.
    \begin{theorem}\label{th:minimax_classification}
        Let $\cdl$ be defined by \eqref{eq:cdl_def}. 
	        \begin{equation}\label{eq:minimax_classification}
	           \inf_{f\text{ Borel}}\cprm(f)=\sup_{\substack{\PP_0'\in\Wball \e (\PP_0)\\ \PP_1'\in \Wball \e (\PP_1)}}\cdl(\PP_0',\PP_1')
	        \end{equation}
	        and furthermore equality is attained for some Borel measurable $\hat f$ and $\hat \PP_1,\hat \PP_0$ with $W_\infty(\hat \PP_0,\PP_0)\leq \e$ and $W_\infty(\hat \PP_1,\PP_1)\leq \e$.
	        
    \end{theorem}
        The first to show such a theorem was \citet{PydiJog2021}. In comparison to their Theorem 8, Theorem~\ref{th:minimax_classification} removes the assumption that $\PP_0,\PP_1$ are absolutely continuous with respect to Lebesgue measure and shows that the minimizer $f^*$ is in fact Borel. We prove this theorem in Appendix~\ref{app:minimax_classification_proof}.
    \citet{Frank2022Existence} prove a similar statement for the surrogate risk $R_\phi^\e$ in Theorem~6. This time, the dual objective is
    \begin{equation}\label{eq:dl_def}
        \dl(\PP_0',\PP_1')
    \end{equation}
    where $C_\phi^*$ is given by \eqref{eq:C_phi_def}.
    \begin{theorem}\label{th:minimax}
            Assume that Assumption~\ref{as:phi} holds, and define $\dl$ by \eqref{eq:dl_def}.
	        
	        \begin{equation}\label{eq:minimax}
	            R_\phi^{\e,*}=\inf_{f \text{ Borel}} \prm(f)=\sup_{\substack{\PP_0'\in\Wball \e (\PP_0)\\ \PP_1'\in \Wball \e (\PP_1)}}  \dl(\PP_0',\PP_1')   
	        \end{equation}
	        and furthermore equality is attained for some Borel measurable $f^*$ and $\PP_1^*,\PP_0^*$ with $W_\infty(\PP_0^*,\PP_0)\leq \e$ and $W_\infty(\PP_1^*,\PP_1)\leq \e$.
	    \end{theorem}
        


    See \citep{PydiJog2021} and \citep{Frank2022Existence} for a further discussion of these results.
    

    
